Advanced Deep Learning Architectures for Accurate Detection of Subsurface Tile Drainage Pipes from Remote Sensing Images

Subsurface tile drainage pipes provide agronomic, economic and environmental benefits. By lowering the water table of wet soils, they improve the aeration of plant roots and ultimately increase the productivity of farmland. They do however also provide an entryway of agrochemicals into subsurface water bodies and increase nutrition loss in soils. For maintenance and infrastructural development, accurate maps of tile drainage pipe locations and drained agricultural land are needed. However, these maps are often outdated or not present. Different remote sensing (RS) image processing techniques have been applied over the years with varying degrees of success to overcome these restrictions. Recent developments in deep learning (DL) techniques improve upon the conventional techniques with machine learning segmentation models. In this study, we introduce two DL-based models: i) improved U-Net architecture; and ii) Visual Transformer-based encoder-decoder in the framework of tile drainage pipe detection. Experimental results confirm the effectiveness of both models in terms of detection accuracy when compared to a basic U-Net architecture. Our code and models are publicly available at https://git.tu-berlin.de/rsim/drainage-pipes-detection.

==> content/old_sections/abstract.tex <==
Subsurface tile drainage pipes provide agronomic, economic and environmental benefits. By lowering the water table of wet soils, they improve the aeration of plant roots and ultimately increase the productivity of farmland. They do however also provide an entryway of agrochemicals into subsurface water bodies and increase nutrition loss of soils. For maintenance and infrastructural development, accurate maps of tile drainage pipe locations and drained agricultural land are needed. However, for multiple reasons, these maps are often outdated or not present. To overcome these restrictions different remote sensing image processing techniques have been applied over the years with varying degrees of success.
Recent developments in deep learning (DL) techniques improve upon the conventional techniques with machine learning segmentation models. In this study, we introduce two DL-based models: i) improved U-Net architecture; and ii) Visual Transformer in the framework of the tile drainage pipe detection. Our research shows that both models can improve the results in the dice coefficient and the \ac{IoU} over the baseline resulting in a dice coefficient of 0.68 and 0.70 for the improved U-Net and the Visual Transformer and an \ac{IoU} of 0.80 and 0.81 respectively.

==> content/old_sections/conclusion.tex <==
In this paper, we have investigated two DL-based models in the context of drainage pipe detection by using remote sensing images. We were able to train reliable models, improving the previous state-of-the-art proposed in Ref.~\citenum{song2021detecting} with regard to the dice coefficient and IoU as defined earlier. It should however again be mentioned, that the authors of Ref.~\citenum{song2021detecting} did not provide a trained model and only a slightly less performative one could be trained to produce these values. 
Regarding $L_{Dice}$, the baseline model as described in Ref.~\citenum{song2021detecting} still performed best. The TransUNet was the best performing model in the experiment with regards to the dice coefficient and the \ac{IoU}. It does however contain a hundred times the parameters of the next best performing model -- the improved U-Net -- and thus takes much longer to train while only offering a small improvement. The decision of which model to use is therefore a question of the use case and the resources available. By adapting new and even more complex models to the task the performance on the existing dataset may still be optimized. However, significant improvements in the prediction quality and especially the generality of the models could be achieved by incorporating more diverse data sets of different domains or at different conditions. This could be used to explore how the existing and new models behave under different settings and whether the soil conditions required for image acquisition mentioned in Ref.~\citenum{song2021detecting} could be improved or made less restrictive.

Apart from the pixel-level metrics we proposed a new way to evaluate the models based on patch-wise thresholding. We introduced a measurement for the applicability of models in real world scenarios, where not the exact position of a drainage pipes is of interest, but the knowledge if a certain area is drained and if so, to what extent. For all but the 'high' class, the improved U-Net and the TransUNet outperform the baseline model with regard to the precision and recall, again highlighting the good performance of the two models newly introduced to the task of drainage pipe detection.

==> content/old_sections/experimental_results.tex <==
% ====== EXPERIMENTAL SETUP ======
% Data set
In the experiment we trained and evaluated the baseline, the improved U-Net and the TransUNet model on the same data set. The data set was initially introduced together with the baseline model in Ref.~\citenum{song2021detecting}. It contains 513 images, separated into 256 training images --  augmented to a total of 3072 -- and 257 validation images. 
The images have 256$\times$256 pixels with a spacial resolution of 30 cm and three channels (RGB). The study site is located near Sunbury, Ohio, USA. The images were obtained using Google Earth. The ground truth images were generated through manual annotation \cite{song2021detecting}.

% Baseline model
The baseline model consists of a basic U-Net architecture with skip connections added, to allow residual learning, consisting of around 0.5 million parameters. More detailed information can be found in Ref.~\citenum{song2021detecting}. 
As no trained model was provided by the authors it was retrained by us using the original code, with only a slight adaption to the computation of $L_{Dice}$ to make the training more stable and allow for better comparability with the newly introduced models. 
The baseline model was trained for 500 epochs with early stopping on the validation loss and 50 epochs patience, until it reached a training loss of 0.37 and a validation loss of 0.46.

% Experimental setup improved U-Net
The learning rate of the improved U-Net was reduced by half every 16 epochs (instead of every 5 epochs as proposed in Ref.~\citenum{augustauskas2020improved}) starting with a learning rate of 0.001. It was trained for 100 epochs \footnote{The best training loss was reached after 93 epochs.} and contains roughly one million parameters.

% Experimental setup TransUNet
The TransUNet was trained for a total of 150 epochs with batch size 24. The learning rate was calculated as $lr = 0.01 \cdot (1 - \frac{i}{E})^{0.9}$, where $E$ notates the maximum epoch 150 and $i$ notates the current epoch. The Transformer backbone was pretrained with an ResNet-50 ViT-B/16 hybrid model on ImageNet\cite{deng2009imagenet}. As a loss function a combination fo 50\% $L_{Dice}$ and 50\% cross entropy loss was used. The full model contains 105 million parameters.

% IoU and Dice coefficient
To compare the performance of the different models, the \ac{IoU} and the Dice coefficient are used. The Dice coefficient is used as defined in Ref.~\citenum{dice1945measures}\footnote{Note that the Dice coefficient differs from the dice loss $L_{Dice}$ mentioned earlier.}. For both the \ac{IoU} and the dice coefficient a threshold needs to be applied before the computation. As done in the implementation of the baseline model in Ref.~\citenum{song2021detecting}, the results are computed by applying all the thresholds in the range from 0.1 to 0.95 in steps of 0.05 and averaging the results.
% Precision, recall, confusion matrix
The dice coefficient and the \ac{IoU} however are sensitive to even small displacements in the prediction, as they compute a pixel-level scoring. Placing a drainage pipe of exactly the right length and orientation at a small offset to the actual position, so that the prediction is exactly parallel to the ground truth with no overlap, will for example result in a dice coefficient and an \ac{IoU} of 0.0. In practice the result however may still be of use, as it shows, that a drainage pipe is located within a certain area.
To evaluate the performance of the models in use cases where not the exact location of drainage pipes is of interest, but only the information if a certain area is drained or not, we introduce new measures. For that the 256$\times$256 binary ground truth and output images are transformed to 3$\times$3 images. 
The resulting 9 patches are classified into 'none', 'low', 'middle' and 'high', indicating the amount of drainage in the patch, by applying thresholds on the amount of positive pixels within a patch. The thresholds are set, based on the deviation of the amount of positive pixels in all ground truth images containing any positive pixels. The threshold for a pixel to be interpreted as positive is set to 0.5.
A transformation of a high resolution ground truth image to a low resolution image can be seen in \cref{fig:high_low_conv}. By a patch-wise comparison of the resulting ground truth and output images, a confusion matrix can be computed and based on that precision and recall values can be determined for the four different classes.
% Move the following to motivation or conclusion?
%The dice coefficient and the \ac{IoU} are sensitive to even small displacements in the prediction, as they compute a pixel-level scoring. Placing a drainage pipe of exactly the right length and orientation at a small offset to the actual position, so that the prediction is exactly parallel to the ground truth with no overlap, will for example result in a dice coefficient and an \ac{IoU} of 0.0. In practice the result however may still be of use, as it shows, that a drainage pipe is located within a certain area. Classifying whole patches with 'none', 'low', 'middle' and 'high' drainage based on the amount of positive pixels can therefore represent real world requirements more accurately for some applications.\\


\def \predictionTableImageWidth {0.16} % define width of individual image here
\def \evaluationImageWidth {0.64} % this is 4x the above

\begin{figure}
\centering
\begin{subfigure}{0.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\evaluationImageWidth\linewidth]{v_261_y.png}  
  \caption{HR Ground Truth (256$\times$256, 8bit grayscale)}
  \label{sfig:hr_gt}
\end{subfigure}
\hspace{15pt}
\begin{subfigure}{0.33\columnwidth}
  \centering
  % include first image
  \includegraphics[width=\evaluationImageWidth\linewidth]{v_261_qr.png}  
  \caption{LR ground truth used for evaluation (3$\times$3, 2bit grayscale)}
  \label{sfig:lr_gt}
\end{subfigure}
\caption{Conversion from High Resolution (HR) Ground Truth to Low Resolution (LR) Ground Truth.}
\label{fig:high_low_conv}
\end{figure}

% ==================== SWITCH between normal and booktabls table ======================= 
\newcommand{\tablemode}{booktabs} % "normal" or "booktabs"

\input{content/tables/\tablemode/dice_iou}
\input{content/tables/\tablemode/pr_comp}

% ====== RESULTS ======
The quantitative results of the experiments can be seen in \cref{tab:dice_iou}. The baseline model reaches the best validation loss of the three models. In both the dice coefficient and the \ac{IoU} however the two newly adapted models surpass the baseline model, with the TransUNet being the best model for both metrics by a small margin. Qualitative results can be seen in \cref{fig:prediction_matrix}. 
The first image shows an example, where all the models create a near-perfect prediction. All the models are in that case able to distinguish between the drainage pipe and the road, even though they both appear as a straight line in the image. 
The second image shows a tendency of the improved U-Net to produce scattered lines. The drainage pipe running diagonally through the top left corner of the image is detected only partially. The TransUNet detects this drainage pipe in its full length. Instead of missing small parts of the drainage pipe it actually predicts very small features, where there should not be any. The baseline model fails to detect this drainage pipe completely. 
In the third image all models have some false positive predictions, detecting a drainage pipe where there should not be one. The surface feature producing the false positive is however hard to distinguish from a feature actually caused by a drainage pipe, even for the human eye. Again it can be seen, that the TransUNet detects the drainage pipe continuously in their full length compared to the baseline and the improved U-Net, but also shows a little more false positives.

For the first time in this work we also evaluate the drainage pipe detection models based on a patch-level classification. The confusion matrices of the different models and a comparison of the precision and recall can be seen in \cref{tab:pr_comp} and \ref{tab:cms}.
Both the improved U-Net and the TransUNet perform well for the none, low and middle class. For those three classes both the precision and the recall lay above 62\%. For the baseline model however the precision and recall in some cases are below 50\%. Only for the high class, all models perform poorly.
This might be related to the low frequency with which the label appears in the data set. For all the models however it can be seen, that usually the prediction is not 'too far off', meaning that patches, that are actually highly drained, that are not detected as high by the network, in the most cases get classified as middle. Similarly patches that where wrongly classified as high, are usually in the middle class.

\begin{figure*}[b]
    \centering
    \begin{tabular}{ccccc}
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/1/rgb_1.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/1/gt_1.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/1/song_1.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/1/unet_1.png}} & 
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/1/vt_1.png}} \\
      %
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/2/rgb_2.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/2/gt_2.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/2/song_2.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/2/unet_2.png}} & 
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/2/vt_2.png}} \\
      %
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/3/rgb_3.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/3/gt_3.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/3/song_3.png}} &
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/3/unet_3.png}} & 
      \addheight{\includegraphics[width=\predictionTableImageWidth\linewidth]{prediction_stack/3/vt_3.png}} \\
      %
      \footnotesize (a) & (b) & (c) & (d) & (e)
    \end{tabular}
    \caption{(a) Aerial images; (b) their ground truth maps; and the prediction maps obtained by using (c) U-Net; (d) improved U-Net; and (e)TransUNet}
    \label{fig:prediction_matrix}
\end{figure*}

\input{content/tables/\tablemode/cms}

==> content/old_sections/intro.tex <==
% What are drainage pipes? Why is it of interest to find them?
Subsurface tile drainage pipes are an essential agricultural element, maintaining or improving water management and crop yields of farm land. Depending on location and respective hydro-climatological conditions, significant parts of farm land are equipped with tile drainage systems (e.g. in Denmark $\sim50\%$ of the agricultural area \cite{Motarjemi2021drainage_mla}). Multiple installation patterns of subsurface drainage system are in use like herringbone, double main, parallel, targeted and complex patterns (see review by Ref.~\citenum{koganti2020mapping} for more information).
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{drainage_pipes.png}
    \caption{Function of drainage pipes and the impact on soil color on the surface (modified from \cite{song2021detecting})}
    \label{fig:drainage_pipes2}
\end{figure}
Besides their positive effects, subsurface drainage pipes also boost -- in high pulse-like signals -- nutrient and pesticide loss of soils with short retention time to surface waters. Especially in areas where surface runoff cannot reach receiving waters and infiltrates into depressions, macropore transport to tile drainage pipes was shown as a dominant pesticide loss pathway of agrochemicals into surface water bodies \cite{Leu2004herbicideloss}, posing risk to both human and ecosystem health. In order to improve the understanding of agro-chemical dynamics in soils, to calculate tile drainage catchment areas and loads for wetland dimension planning, as well as to prepare reliable eco-hydrological models, it is thus crucial to identify the location of drainage pipes \cite{DeSchepper2017drainag_model}. One typical example for parallel tile drainage pipes in flat lowland regions is depicted in \cref{fig:drainage_pipes2}. The pipes are roughly ten centimeters in diameter and installed at about one meter below surface \cite{song2021detecting}. Precipitation (at $t_0$) infiltrates rapidly through the soil above the drainage pipes ($t_1$ and $t_2$) due to preferential flow through especially macropores, leading to relatively low (close to drainage pipes) and relatively high (farther away from the pipes) soil moisture. As the surface albedo increases with decreasing soil moisture, those differences in soil moisture become visible. As shown in \cref{fig:drainage_pipes2}, the soil above the drainage pipes appears brighter after a precipitation event, thus producing distinct features visible at the surface \cite{koganti2020mapping, song2021detecting}.

The lack of documentation of installed drainage pipes has driven researchers to explore other detection methods, such as thermal images and ground-penetrating radar (GPR) \cite {Allred2020thermal}. Their practical applicability is however limited by the restricted data availability. Conventional image processing methods have been applied to remote sensing images of bare soils, obtained after precipitation events \cite{Kratt2020FieldTT}, among them edge detection, decision tree classification and image differencing \cite{gokkaya2017subsurface}. Machine learning techniques are a promising approach to analyse remote sensing data \cite{Cho_2019_ML_drainage, OHara2020_ML_drainage, song2021detecting}. 
% What has so far been done to detect them?
  %TODO: Check sources
In Ref.~\citenum{song2021detecting} a drainage pipe detection approach based on a deep learning U-Net architecture \cite{ronneberger2015u} and remote sensing images was developed. It outperforms other remote sensing image based approaches using edge detection. The authors suggest that even though the model shows good performance, it may still be improved by tuning hyperparameters and using a more diverse training set \cite{song2021detecting}.

In this work however we aim to improve on the results of the model proposed in Ref.~\citenum{song2021detecting}, which will serve as a baseline to compare all obtained results to, by different measures. We newly introduce two DL-based models to the task of drainage pipe detection:  a visual transformer and U-Net architecture with multiple adaptions.


==> content/old_sections/method.tex <==

We adapt two DL-based models to the task of semantic segmentation for tile drainage pipe detection, one based on an improved U-Net and one based on a Visual Transformer. Both models have the goal to predict a pixel-wise mapping $M$ with $x \mapsto M(x)$ where $x \in \mathds{R}^{H\times W\times C}$ and $M(x) \in \mathds{R}^{H\times W\times 1}$. The mapping function is trained by minimizing the dice loss function $L_{Dice}$ as defined in Ref.~\citenum{song2021detecting}. The details of each method are presented in the following subsections.
%\todo{add out metric here, but it does not seem very intuitive to add it here?}

\begin{figure}
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.8\columnwidth]{ImprUNet_arch_compact.jpg}
    \caption{The improved U-Net architecture is based on a four-layer U-Net consisting of an encoder and a decoder part and is enhanced with residual blocks, \ac{AG} and \ac{ASPP} modules. The 'bottleneck' is the most contracted part with the highest number of convolutional kernels. (based on:  Ref.~\citenum{augustauskas2020improved})}
    \label{fig:improved_unet_architecture}
\end{subfigure}
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=.8\columnwidth]{TransUNet_arch_compact.jpg}
    \caption{Design of the TransUNet network: A CNN is used for low level feature extraction, followed by a Transformer Encoder for high level features. To improve the location accuracy of the upscaling decoder, skip connections are added from the CNN to the decoder layers. (based on: Ref.~\citenum{chen2021transunet})}
    \label{fig:transunet_arch}
\end{subfigure}
\caption{Architectures of the introduced models: Both models take as input an image with $C$ channels and a $H\times W$-resolution and output a grayscale image of the same resolution. The gray value of a pixel in the output represents the probability of a drainage pipe being in the location of that pixel. }
\label{fig:architectures}
\end{figure}

\subsection{Improved U-Net}\label{ssec:unet}
The U-Net architecture was introduced in Ref.~\citenum{ronneberger2015u} for the task of biomedical image segmentation. It contains a contracting and an expansive path. The contracting path captures context, whereas the expanding path allows precise localization. Both paths are in a way symmetric to each other. 
%he contracting path consists  of a series of convolutions -- each followed by a \ac{ReLU} -- and max-pooling operations, doubling the number of feature channels in every downsampling step. The expansive path consists of  a series of upsampling, convolution and \ac{ReLU} operations, halfing the number of feature channels in every step while using a concatenation with the feature map of the contracting path.
This fully convolutional auto-encoder-decoder networks (FCN) can be trained with very few images. FCNs demonstrate good performance in different biomedical segmentation applications \cite{ronneberger2015u}, and other complicated computer-vision image segmentation tasks \cite{augustauskas2020improved}.

In Ref.~\citenum{augustauskas2020improved} multiple U-Net architectures with several adaptions are introduced, improving the image segmentation performance without significant computational overhead. In this work we introduce one of the proposed candidates to the task of drainage pipe detection. As it is based on a U-Net architecture, but incorporates several additions, it is in the following denoted as the 'improved U-Net'. Its architecture can be seen in \cref{fig:improved_unet_architecture}. At its core is a four-layer U-Net using 3$\times$3 kernels and a stride of one for all convolutions. Padding was added, so that input and output dimensions match and batch normalization was added between each convolutional layer and its activation function (except for the last output layer), to make the network more stable. 
The main architectural changes with regard to the original U-Net architecture are i) added residual connections, ii) \ac{ASPP} and iii) \ac{AG} modules \cite{augustauskas2020improved}.
Residual learning addresses the degradation problem, which occurs when the performance of a network degrades with increasing depth, by introducing shortcut connections, skipping one ore more layers. Residual blocks thus allow to gain accuracy through increased depth, while being easy to optimize \cite{he2015deep}.
In the \ac{ASPP} module a sequence of convolutions with different dilation rates is performed \cite{augustauskas2020improved}. The dilated convolutions allow to expand the receptive field without losing resolution. A module using dilated convolutions is thus able to extract multi-scale information \cite{yu2016multiscale}.
The \ac{AG} modules learn to focus on the target structure without the need of further supervision \cite{schlemper2019attention}. % TODO: change wording.
In this way they highlight important features, while suppressing irrelevant ones \cite{augustauskas2020improved}.
More detailed information on residual blocks, the \ac{ASPP} and \ac{AG} modules and the way they are combined together in the improved U-Net model can be found in \cite{he2015deep, augustauskas2020improved, yu2016multiscale, schlemper2019attention}.  
Detecting tile drainage pipes from RGB remote sensing images using a deep U-Net architecture was proposed in Ref.~\citenum{song2021detecting}. However, this U-Net architecture is simple and cannot utilize multiscale contexts in the latent space at the bottleneck or emphasize relevant and deemphasize irrelevant information in the residual connections. These problems are addressed in the improved U-Net used in this paper.
    
\subsection{Visual Transformer} \label{ssec:vt}
In Ref.~\citenum{dosovitskiy2020image} an architecture based on Transformers \cite{vaswani2017attention} like used in state-of-the-art \ac{NLP} is proposed. This architecture divides a given problem into a sequence of tokens and processes it via a stack of combinations of an multi-head attention layer similar to what was described in \cref{ssec:unet} and a fully connected layer. 
When dividing the image into small patches the image $x$ can be described as a sequence of $N$ non-overlapping patches $\{x_p^i \in \mathds{R}^{P^2\cdot C} | i = 1, \dots, N\}$ with patch size $P \times P$ and $N = \frac{HW}{P^2}$ patches\footnote{Number of patches is equal to the length of the input sequence.}. 
Parts of the patches are weighted using multiple attention heads, where the patches are treated like in a sequence problem. The fully connected layer combines these weighted results in combination with residual connections to produce higher level features. 
This encoder architecture is refined with skip connections to retain low level features for tasks like segmentation as Chen et al. propose in Ref.~\citenum{chen2021transunet}. This results in a UNet-like architecture. 
The skip connections are inserted between the patch encoders and the upscaling layers. Additionally this work applies some simple convolutions in patch Encoder part as can be seen in \cref{fig:transunet_arch}. 
The feature maps of the convolutions are the input of the encoder and additionally directly connected to the upscaling decoder of high level feature maps created by the Vision Transformer encoder. 
This results in the decoder being able to combine high level features form the Transformer Encoder and low level features from the convolutions.

Very deep networks for transfer learning as used in their state-of-the-art form tend to take a long time when trained on a large data set, but they develop great generalisation capabilities if the data set is diverse as shown in Ref.~\citenum{kolesnikov2019big}. Visual Transformers are significantly faster than convolutional networks as shown in Ref.~\citenum{vaswani2017attention}, however they still take very long to train. Therefore using pretrained weights and only fine tuning the networks is the approach taken in this work for the TransUNet model.

==> content/tables/normal/cms.tex <==
\begin{table}
\centering
    \begin{tabular}{|l||l|c|c|c|c|}
        \hline
         model & \diagbox{GT}{pred.} &   None    &   Low     &   Middle  &   High    \\\hline
         \multirow{4}{*}{Baseline} & None   &   1433    &   185     &   19      &   0       \\\cline{2-6}
                                   & Low    &   33      &   181     &   154     &   4       \\\cline{2-6}
                                   & Middle &   22      &   26      &   180     &   45      \\\cline{2-6}
                                   & High   &   2       &   5       &   14      &   10      \\
         \hline
         \multirow{4}{*}{Impr. U-Net} & None   &   1530    &   105     &   2       &   0       \\\cline{2-6}
                                   & Low    &   16      &   301     &   55      &   0       \\\cline{2-6}
                                   & Middle &   6       &   74      &   185     &   8      \\\cline{2-6}
                                   & High   &   1       &   6       &   20      &   4      \\
         \hline
         \multirow{4}{*}{TransUNet} & None   &   1539    &   92      &   6       &   0       \\\cline{2-5}
                                   & Low    &   15      &   288     &   69      &   0       \\\cline{2-6}
                                   & Middle &   6       &   65      &   198     &   4     \\\cline{2-6}
                                   & High   &   1       &   4       &   17      &   9       \\
         \hline
    \end{tabular}
    \label{tab:cms}
    \caption{Confusion matrices of the different models }
\end{table}

==> content/tables/normal/dice_iou.tex <==
\begin{table}[b]
    \centering
    \caption{$L_{Dice}$, dice coefficient and \ac{IoU} of the three different models on validation set of the data set provided in \cite{song2021detecting}.}
    \label{tab:dice_iou}
    \normalsize
    \begin{tabular}{|l|c|c|c|}
        \hline
        \textbf{model} & \textbf{$L_{Dice}$} &\textbf{Dice coefficient} & \textbf{\ac{IoU}} \\
        \hline
        Baseline & \textbf{0.46} & 0.55 & 0.76 \\
        \hline
        Impr. U-Net & 0.79 & 0.68 & 0.80 \\
        \hline
        TransUNet & 0.79 & \textbf{0.70} & \textbf{0.81} \\
        \hline
    \end{tabular}
\end{table}

==> content/tables/normal/pr_comp.tex <==
\begin{table}
    \centering
    \normalsize
    \begin{tabular}{| l | l | c | c |}
        \hline
         \textbf{model} & \textbf{class} & \textbf{precision} & \textbf{recall}\\\hline
         
         \multirow{4}{*}{Baseline} & none & 0.96 & 0.88 \\\cline{2-4}
         & low & 0.46 & 0.49 \\\cline{2-4}
         & middle & 0.49 & 0.65 \\\cline{2-4}
         & high & 0.17 & \textbf{0.32} \\\hline
         
         \multirow{4}{*}{Impr. U-Net}& none & \textbf{0.99} & 0.93 \\\cline{2-4}
         & low & 0.62 & \textbf{0.81} \\\cline{2-4}
         & middle & \textbf{0.71} & 0.68 \\\cline{2-4}
         & high & 0.33 & 0.13 \\\hline
         
         \multirow{4}{*}{TransUNet}& none & \textbf{0.99} & \textbf{0.94} \\\cline{2-4}
         & low & \textbf{0.64} & 0.77 \\\cline{2-4}
         & middle & 0.68 & \textbf{0.72} \\\cline{2-4}
         & high & \textbf{0.69} & 0.29 \\\hline
    \end{tabular}
    \caption{Precision and recall of the different classes for the different models.}
    \label{tab:pr_comp}
\end{table}
